Hate is the New Infodemic: A Topic-aware Modeling of Hate Speech Diffusion on Twitter

Online hate speech, particularly over microblogging platforms like Twitter, has emerged as arguably the most severe issue of the past decade. Several countries have reported a steep rise in hate crimes infuriated by malicious hate campaigns. While the detection of hate speech is one of the emerging research areas, the generation and spread of topic-dependent hate in the information network remain under-explored. In this work, we focus on exploring user behaviour, which triggers the genesis of hate speech on Twitter and how it diffuses via retweets. We crawl a large-scale dataset of tweets, retweets, user activity history, and follower networks, comprising over 161 million tweets from more than $41$ million unique users. We also collect over 600k contemporary news articles published online. We characterize different signals of information that govern these dynamics. Our analyses differentiate the diffusion dynamics in the presence of hate from usual information diffusion. This motivates us to formulate the modelling problem in a topic-aware setting with real-world knowledge. For predicting the initiation of hate speech for any given hashtag, we propose multiple feature-rich models, with the best performing one achieving a macro F1 score of 0.65. Meanwhile, to predict the retweet dynamics on Twitter, we propose RETINA, a novel neural architecture that incorporates exogenous influence using scaled dot-product attention. RETINA achieves a macro F1-score of 0.85, outperforming multiple state-of-the-art models. Our analysis reveals the superlative power of RETINA to predict the retweet dynamics of hateful content compared to the existing diffusion models.

==> viz_tool.tex <==
% In addition, we develop \viztool, an open-source tool to visualize, inspect, and compare diffusion dynamics over networks.

% \item We present \viztool\ (\viztoolexpand), an open-source tool to visualize diffusion over social and information networks. We incorporate multiple diffusion models and showcase the outputs of \viztool\ in Section~\ref{sec:viz_tool}.

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.95\textwidth]{Figures/viz_tool.pdf}
%     \caption{{\bf A screenshot of diffusion dashboard for \viztool.} This is the main window for visualizing diffusion. The screenshot shows the state of graph at iteration 27, using the profile threshold diffusion algorithm.}
%     \label{fig:viz_tool}
%     \vspace{-5mm}
% \end{figure*}

% \section{\viztool: A Diffusion Visualization tool}
% \label{sec:viz_tool}
% There are many tools for visualizing graphs, such as NetworkX\cite{aric_networkx_11} and Gephi\cite{bastian2009gephi}. Unfortunately, they are difficult to customize for visualization and cannot interactively monitor streaming data. On the other hand, there are tool-kits\cite{ToolkitViz} that visualize certain aspect of the Twitter data like topical \cite{TopicViz} or sentiment\cite{SentiCompass},\cite{Sent_Viz}  alignments. Inspired by the likes of Twitter Visualization\footnote{\protect\url{https://www.csc2.ncsu.edu/faculty/healey/tweet_viz/}}, we have created a web toolkit, called \viztool\ (\viztoolexpand), designed specifically for the exploration and analysis of diffusion algorithms in social networks. It is built on an open-source library, VivaGraphJS\footnote{\protect\url{https://github.com/anvaka/VivaGraphJS}}. Figure \ref{fig:viz_tool} shows a screenshot of \viztool. 

% \subsection{Input}
% The tool builds a directed graph from a simple JSON file of the edge list. For eg., given a JSON of network $\{u : [v,w], v: [z]\}$, the edge list in the network will be $\{(u,v), (u,w), (v,z)\}$, where, for the tuple $(u,v)$,  the edge will be directed from $u$ to $v$. The imported network can be a real or a mock social network. Nodes can be profiled with names, images, etc. While we are using Twitter networks, any social network compiled in the same format can be imported.

% A node has three components: the id or name as a label, the profile data displayed on clicking the node and the edges to the connected nodes. Each link stores the id of the nodes it connects.

% Once a network is loaded, it is clustered using a label propagation algorithm included in the ngraph\footnote{\protect\url{https://github.com/anvaka/ngraph}} library. These clusters can be interpreted as social groups or communities, essentially allowing visual diffusion between groups.


% \subsection{Usage}
% The tool creates an interactive graph and analysis of diffusion from the input. It can be used for simulating a diffusion or visualizing an existing diffusion. The graph shows diffusion by changing the color of nodes and edges to red as they become ``infected" or are tagged as re-tweeters in a series of single hops, i.e., one iteration or unit-time. 

% For simulation, the seed nodes can be selected after clicking on them. The baseline algorithms discussed in the paper have been included in the tool for simulation. They are included as external APIs which allow usage of custom diffusion algorithms by creating APIs which support the same format.

% For visualizing an existing diffusion, the cascade can be compiled into a simple JSON file. A cascade for one user is a list of re-tweeters at each iteration(timestamp).

% Let us assume a diffusion as follows: $\{
% u: [[v,w], [z]],\ 
% x: [[\ ], [y]]
% \}.$, where nodes $u$ and $x$ post some content at time $t = t_0$. At time $t = t_1$, the nodes $\{ u, v, w, x\}$  and the edges $\{(u,v), (u,w)\}$ will be red. At time $t = t_2$, the nodes $\{ u, v, w, x, y, z\}$ and the edges $\{(u,v), (u,w), (u,z), (x,y)\}$ will be red. 

% \viztool\ also provides interactive plots for some statistics related to the diffusion, including temporal growth of re-tweeters or infected nodes, and temporal growth of susceptible nodes.

% To our knowledge, \viztool\ will be the first open-source diffusion visualization tool with several customization options for users, including new networks, new diffusion models, visualizing the ground-truth, and comparing it with the model outputs.

% Adding to these mentioned contributions, we also developed \viztool, an open-source library for visualizing diffusion over social and information networks. 
